Improving Zero-shot Generalization in Offline Reinforcement Learning using Generalized Similarity Functions

Reinforcement learning (RL) agents are widely used for solving complex sequential decision making tasks, but still exhibit difficulty in generalizing to scenarios not seen during training. While prior online approaches demonstrated that using additional signals beyond the reward function can lead to better generalization capabilities in RL agents, i.e. using self-supervised learning (SSL), they struggle in the offline RL setting, i.e. learning from a static dataset. We show that performance of online algorithms for generalization in RL can be hindered in the offline setting due to poor estimation of similarity between observations. We propose a new theoretically-motivated framework called Generalized Similarity Functions (GSF), which uses contrastive learning to train an offline RL agent to aggregate observations based on the similarity of their expected future behavior, where we quantify this similarity using \emph{generalized value functions}. We show that GSF is general enough to recover existing SSL objectives while also improving zero-shot generalization performance on a complex offline RL benchmark, offline Procgen.

==> 6_analysis.tex <==

In this section, we show that the number of quantile bins used by \shortmethod{} follows a bias-variance trade-off, and has to be picked based on POMDP specifics.
% Contributions of this section are as follows:
% \begin{enumerate}
%     \item We highlight a trade-off in the extrapolation erorr that occurs for the number of bins $K$.
%     \item We show that optimizing $\ell_
%     \text{NCE}$ over samples by $\mu$ from $M_i,M_j$ for the case of successor features norm amounts to minimizing the interpolation error of the representation over $\cD^\mu$.
%     \item We show how action-based distances similar to those in prior works~\citep{liu2020cross,agarwal2021contrastive} can be recovered within our framework.
% \end{enumerate}


% \begin{theorem}
% Let $f$ be an encoder such that $\nabla \ell_{NCE}(\theta_h,\psi,\mat{W})\approx 0$. Then, for any $o_1\in M_1, o_2\in M_2$ and $p\in (0,1)$ s.t. $o_1,o_2\in I(p)$, the following holds:
% $$|V^\mu(\vec{s}_1)-V^\mu(\vec{s}_2)|<C|G^\mu_1(\vec{s}_1)-G^\mu_2(\vec{s}_2)|$$
% \bogdan{TODO}
% \label{thm:value_bound}
% \end{theorem}

% Recall that the error made by a simple TD estimator $\hat{G}^\mu$ is accumulated over future timesteps and scaled by $\sup_{\vec{s}\in\cS}c(s)$~\citep{su2020adaptive}:
% \begin{equation}
%   |\mathbb{E}_{z\sim \mathbb{P}^\mu_t}[G^\mu(\vec{s}_t)-\hat{G}^\mu(\vec{s}_t)]|<\frac{\gamma^t-\gamma^T}{1-\gamma}\sup_{\vec{s}\in\cS}c(s)=\delta_c(t;\gamma,T)
% \end{equation}
Thm.~\ref{thm:gvf_bound} highlights a trade-off when choosing the number of quantiles bins empirically.
\begin{theorem}
Let $G_1$, $G_2$ be generalized value functions with cumulants $c_1,c_2$ from respective POMDPs $M_1,M_2$, $K$ be the number of quantile bins, $n_1,n_2$ the number of sample transitions from each POMDP. Suppose that $\mathbb{P}[\sup_{t=1,2,..}|c_1(o_{1,t},\mu(o_{1,t}))-c(o_{2,t},\mu(o_{2,t}))|>\nicefrac{(1-\gamma)\varepsilon}{\gamma}]\leq \delta$. Then, for any $k=1,..,K$ and $\varepsilon>0$ the following holds
\begin{equation}
    \begin{split}
       \mathbb{P}[ \sup_{o_1,o_2\in I(k)}|G_1(o_1)-G_2(o_2)| > 3\varepsilon]
        &\leq Ce^{-2n_i\varepsilon^2/4}+p(n_i,K,\varepsilon)+\delta \\ 
    \end{split}
\end{equation}
where
\begin{equation}
    p(n_i,K,\varepsilon)=\mathbb{P}[\sup_{k\in [1,K]}\big|\hat{F}^{-1}_{i}\big(\frac{k+1}{K}\big)-\hat{F}^{-1}_{i}\big(\frac{k}{K}\big)\big|>\varepsilon]
\end{equation} and some constant $C>0$.
\label{thm:gvf_bound}
\end{theorem}

All proofs can be found in the Appendix Sec.~\ref{sec:proofs}. For POMDP $M_1$, the error decreases linearly with increasing bin number $K$ (second term).
However, the variance of bin labels directly depends on the number of sample transitions $n_1$ (first term). The inter-POMDP error (third term) does not affect the bin assignment. Hence, choosing a large $K$ will amount to pairing states by rankings, but results in high variance, as orderings are estimated from data and each bin will have $n=1$. Setting $K$ too small will group together undesirable observations, inducing high bias.

Thm.~\ref{thm:sf_bound} can be found in the Appendix and demonstrates that using successor features as GVF amounts to grouping observation representations by their visitation counts - a heuristic which results in lower interpolation error for bin $I(K)$ due to higher sample size.


% First, note that
% \begin{equation}
%     \begin{split}
%         ||G^\mu(\vec{s}_1,a)-G^\mu(\vec{s}_2,a)||_1 &= ||\theta^\top_a(f(\vec{s}_1)-f(\vec{s}_2))||_1\\
%     &\leq ||\theta^\top_a||_\infty \cdot ||f(\vec{s}_1)-f(\vec{s}_2)||_1 \text{ for } \vec{s}_1,\vec{s}_2\in I(p)
%     \end{split}
% \end{equation}

% It can be shown that,
% \begin{equation}
%     \begin{split}
%         \sup_{p\in}\sup_{\vec{z}_1,\vec{z}_2\in I(p)}\bigg|F^{-1}_{G^\mu_i}\bigg(p+\frac{1}{K}\bigg)-F^{-1}_{G^\mu_i}(p)\bigg|&\leq\sup_{\vec{z}_1,\vec{z}_2\in I(p)}\bigg|F^{-1}_{G^\mu_i}\bigg(p+\frac{1}{K}\bigg)-\hat{F}^{-1}_{G^\mu_i}\bigg(p+\frac{1}{K}\bigg)\bigg|\\
%         &+\bigg|F^{-1}_{G^\mu_i}\bigg(p+\frac{1}{K}\bigg)-F^{-1}_{G^\mu_i}(p)\bigg|\\
%     \end{split}
% \end{equation}


% \textbf{PAC version of bound}
% and for a greedy policy $\pi_{Q^\mu}(\vec{s})=\argmax_{a\in \cA} Q^\mu(\vec{s},a)$,
% \begin{equation}
%     \mathbb{P}[\pi_{Q^\mu}(\vec{s}_1)=\pi_{Q^\mu}(\vec{s}_2)]
% \end{equation}

% The agreement happens iff the encoders map, with high probability, two states $\vec{s}_1,\vec{s}_2\in I(p)$ close in latent space, or
% \begin{equation}
%   \begin{split}
%   \mathbb{P}[|\max_{a\in\cA} Q^\mu(\vec{s}_1,a)-\max_{a\in\cA}Q^\mu(\vec{s}_2,a)|<\varepsilon_p] &=  \mathbb{P}[|| Q^\mu(\vec{s}_1,\cdot)||_\infty-||Q^\mu(\vec{s}_2,\cdot)||_\infty<\varepsilon_p]\\
%         &= \mathbb{P}[||f(\vec{s}_1)-f(\vec{s}_2)||_1 < \varepsilon_p]\\
%         &=1-\mathbb{P}[||f(\vec{s}_1)-f(\vec{s}_2)||_1\geq \varepsilon_p]\\
%         & <1-2e^{\frac{1-(1-\varepsilon_p)^2}{2}}\\
%   \end{split}
% \end{equation}

% The above holds only if $||f(\vec{s}_1)||=||f(\vec{s}_2)||=1/2$.





==> figures/state_action_aliasing.tex <==
\begin{figure}[h!]
    \centering
\tikzset{every picture/.style={line width=0.7pt}} %set default line width to 0.75pt        
\resizebox{.75\textwidth}{!}{
\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,611); %set diagram left start at 0, and has height of 611

%Shape: Circle [id:dp36294346457416804] 
\draw   (193,163) .. controls (193,149.19) and (204.19,138) .. (218,138) .. controls (231.81,138) and (243,149.19) .. (243,163) .. controls (243,176.81) and (231.81,188) .. (218,188) .. controls (204.19,188) and (193,176.81) .. (193,163) -- cycle ;
%Shape: Circle [id:dp8038282382752409] 
\draw   (273,162) .. controls (273,148.19) and (284.19,137) .. (298,137) .. controls (311.81,137) and (323,148.19) .. (323,162) .. controls (323,175.81) and (311.81,187) .. (298,187) .. controls (284.19,187) and (273,175.81) .. (273,162) -- cycle ;
%Shape: Circle [id:dp23618516031960213] 
\draw   (350,163) .. controls (350,149.19) and (361.19,138) .. (375,138) .. controls (388.81,138) and (400,149.19) .. (400,163) .. controls (400,176.81) and (388.81,188) .. (375,188) .. controls (361.19,188) and (350,176.81) .. (350,163) -- cycle ;
%Shape: Circle [id:dp1751539958290127] 
\draw   (273,247) .. controls (273,233.19) and (284.19,222) .. (298,222) .. controls (311.81,222) and (323,233.19) .. (323,247) .. controls (323,260.81) and (311.81,272) .. (298,272) .. controls (284.19,272) and (273,260.81) .. (273,247) -- cycle ;
%Shape: Circle [id:dp7928530267898726] 
\draw   (273,333) .. controls (273,319.19) and (284.19,308) .. (298,308) .. controls (311.81,308) and (323,319.19) .. (323,333) .. controls (323,346.81) and (311.81,358) .. (298,358) .. controls (284.19,358) and (273,346.81) .. (273,333) -- cycle ;
%Straight Lines [id:da5932094131204071] 
\draw    (231.33,185.67) -- (280.8,227.05) ;
\draw [shift={(282.33,228.33)}, rotate = 219.92000000000002] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da9684975616040277] 
\draw    (363.33,185.67) -- (318.44,228.95) ;
\draw [shift={(317,230.33)}, rotate = 316.05] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da31695613268471057] 
\draw    (298,187) -- (298,220) ;
\draw [shift={(298,222)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da6591577482767614] 
\draw    (298,272) -- (298,305) ;
\draw [shift={(298,307)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Shape: Circle [id:dp03076961254184285] 
\draw   (437,160.33) .. controls (437,146.53) and (448.19,135.33) .. (462,135.33) .. controls (475.81,135.33) and (487,146.53) .. (487,160.33) .. controls (487,174.14) and (475.81,185.33) .. (462,185.33) .. controls (448.19,185.33) and (437,174.14) .. (437,160.33) -- cycle ;
%Shape: Circle [id:dp26798316899749586] 
\draw   (517,159.33) .. controls (517,145.53) and (528.19,134.33) .. (542,134.33) .. controls (555.81,134.33) and (567,145.53) .. (567,159.33) .. controls (567,173.14) and (555.81,184.33) .. (542,184.33) .. controls (528.19,184.33) and (517,173.14) .. (517,159.33) -- cycle ;
%Shape: Circle [id:dp30625689640320064] 
\draw   (594,160.33) .. controls (594,146.53) and (605.19,135.33) .. (619,135.33) .. controls (632.81,135.33) and (644,146.53) .. (644,160.33) .. controls (644,174.14) and (632.81,185.33) .. (619,185.33) .. controls (605.19,185.33) and (594,174.14) .. (594,160.33) -- cycle ;
%Shape: Circle [id:dp1550144168201275] 
\draw   (517,244.33) .. controls (517,230.53) and (528.19,219.33) .. (542,219.33) .. controls (555.81,219.33) and (567,230.53) .. (567,244.33) .. controls (567,258.14) and (555.81,269.33) .. (542,269.33) .. controls (528.19,269.33) and (517,258.14) .. (517,244.33) -- cycle ;
%Shape: Circle [id:dp5659640995635111] 
\draw   (517,330.33) .. controls (517,316.53) and (528.19,305.33) .. (542,305.33) .. controls (555.81,305.33) and (567,316.53) .. (567,330.33) .. controls (567,344.14) and (555.81,355.33) .. (542,355.33) .. controls (528.19,355.33) and (517,344.14) .. (517,330.33) -- cycle ;
%Straight Lines [id:da35082708975021104] 
\draw    (462,185.33) -- (461.69,218.67) ;
\draw [shift={(461.67,220.67)}, rotate = 270.54] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da9754489886612048] 
\draw    (619,185.33) -- (618.69,218.67) ;
\draw [shift={(618.67,220.67)}, rotate = 270.54] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da28026841943062974] 
\draw    (542,184.33) -- (542,217.33) ;
\draw [shift={(542,219.33)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da39637301649828083] 
\draw    (542,269.33) -- (542,302.33) ;
\draw [shift={(542,304.33)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Shape: Circle [id:dp007082741899542722] 
\draw   (273,417.33) .. controls (273,403.53) and (284.19,392.33) .. (298,392.33) .. controls (311.81,392.33) and (323,403.53) .. (323,417.33) .. controls (323,431.14) and (311.81,442.33) .. (298,442.33) .. controls (284.19,442.33) and (273,431.14) .. (273,417.33) -- cycle ;
%Straight Lines [id:da5167616437467943] 
\draw    (298,358) -- (298,391) ;
\draw [shift={(298,393)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Shape: Circle [id:dp7988409429888437] 
\draw   (273.67,501) .. controls (273.67,487.19) and (284.86,476) .. (298.67,476) .. controls (312.47,476) and (323.67,487.19) .. (323.67,501) .. controls (323.67,514.81) and (312.47,526) .. (298.67,526) .. controls (284.86,526) and (273.67,514.81) .. (273.67,501) -- cycle ;
%Straight Lines [id:da22003800657398975] 
\draw    (298,442.33) -- (298,475.33) ;
\draw [shift={(298,477.33)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Shape: Circle [id:dp344955707851464] 
\draw   (436.67,245.67) .. controls (436.67,231.86) and (447.86,220.67) .. (461.67,220.67) .. controls (475.47,220.67) and (486.67,231.86) .. (486.67,245.67) .. controls (486.67,259.47) and (475.47,270.67) .. (461.67,270.67) .. controls (447.86,270.67) and (436.67,259.47) .. (436.67,245.67) -- cycle ;
%Shape: Circle [id:dp029840929396911298] 
\draw   (593.67,245.67) .. controls (593.67,231.86) and (604.86,220.67) .. (618.67,220.67) .. controls (632.47,220.67) and (643.67,231.86) .. (643.67,245.67) .. controls (643.67,259.47) and (632.47,270.67) .. (618.67,270.67) .. controls (604.86,270.67) and (593.67,259.47) .. (593.67,245.67) -- cycle ;
%Straight Lines [id:da27626351577482033] 
\draw    (461.67,270.67) -- (461.67,303.67) ;
\draw [shift={(461.67,305.67)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da3441148169951356] 
\draw    (618.67,270.67) -- (618.67,303.67) ;
\draw [shift={(618.67,305.67)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Shape: Circle [id:dp5394621315432471] 
\draw   (437.67,331.67) .. controls (437.67,317.86) and (448.86,306.67) .. (462.67,306.67) .. controls (476.47,306.67) and (487.67,317.86) .. (487.67,331.67) .. controls (487.67,345.47) and (476.47,356.67) .. (462.67,356.67) .. controls (448.86,356.67) and (437.67,345.47) .. (437.67,331.67) -- cycle ;
%Shape: Circle [id:dp8664738296405723] 
\draw   (593.67,331) .. controls (593.67,317.19) and (604.86,306) .. (618.67,306) .. controls (632.47,306) and (643.67,317.19) .. (643.67,331) .. controls (643.67,344.81) and (632.47,356) .. (618.67,356) .. controls (604.86,356) and (593.67,344.81) .. (593.67,331) -- cycle ;
%Shape: Circle [id:dp07132692128852658] 
\draw   (518,414) .. controls (518,400.19) and (529.19,389) .. (543,389) .. controls (556.81,389) and (568,400.19) .. (568,414) .. controls (568,427.81) and (556.81,439) .. (543,439) .. controls (529.19,439) and (518,427.81) .. (518,414) -- cycle ;
%Straight Lines [id:da07894222697464093] 
\draw    (462.67,356.67) -- (524.6,392.66) ;
\draw [shift={(526.33,393.67)}, rotate = 210.16] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da3384378088572919] 
\draw    (542,355.33) -- (542,388.33) ;
\draw [shift={(542,390.33)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da029268756159662734] 
\draw    (618.67,356) -- (562,393.89) ;
\draw [shift={(560.33,395)}, rotate = 326.23] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Shape: Circle [id:dp5961632280058378] 
\draw   (518,498) .. controls (518,484.19) and (529.19,473) .. (543,473) .. controls (556.81,473) and (568,484.19) .. (568,498) .. controls (568,511.81) and (556.81,523) .. (543,523) .. controls (529.19,523) and (518,511.81) .. (518,498) -- cycle ;
%Straight Lines [id:da8093215343126368] 
\draw    (542,439.33) -- (542,472.33) ;
\draw [shift={(542,474.33)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

% Text Node
\draw (211,153) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle o_{1}$};
% Text Node
\draw (289,152) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle o_{2}$};
% Text Node
\draw (366,153) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle o_{3}$};
% Text Node
\draw (293,237) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle z$};
% Text Node
\draw (293,323) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle a$};
% Text Node
\draw (253.33,95) node [anchor=north west][inner sep=0.75pt]   [align=left] {Ideal scenario};
% Text Node
\draw (455,150.33) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle o_{1}$};
% Text Node
\draw (533,149.33) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle o_{2}$};
% Text Node
\draw (610,150.33) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle o_{3}$};
% Text Node
\draw (537,320.33) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle a_{2}$};
% Text Node
\draw (491.33,95.67) node [anchor=north west][inner sep=0.75pt]   [align=left] {Actual scenario};
% Text Node
\draw (293,407.33) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle e$};
% Text Node
\draw (273.67,491) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle Q( z,e)$};
% Text Node
\draw (452.67,235.67) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle z_{1}$};
% Text Node
\draw (534.67,233) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle z_{2}$};
% Text Node
\draw (611.33,234.33) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle z_{3}$};
% Text Node
\draw (457.67,321.67) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle a_{1}$};
% Text Node
\draw (613.67,321) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle a_{3}$};
% Text Node
\draw (538,404) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle e$};
% Text Node
\draw (510.33,488) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle Q( z_{2} ,e)$};
% Text Node
\draw (18,262.67) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle  \begin{array}{{>{\displaystyle}l}}
o:\ observation\\
z:\ latent\ state\\
a:\ action\\
e:\ action\ effect\\
Q:\ state-action\ value\ function
\end{array}$};
\end{tikzpicture}}
\caption{Caption}
    \label{fig:my_label}
\end{figure}
